SciNews: From Scholarly Complexities to Public Narratives -- A Dataset for Scientific News Report Generation

Scientific news reports serve as a bridge, adeptly translating complex research articles into reports that resonate with the broader public. The automated generation of such narratives enhances the accessibility of scholarly insights. In this paper, we present a new corpus to facilitate this paradigm development. Our corpus comprises a parallel compilation of academic publications and their corresponding scientific news reports across nine disciplines. To demonstrate the utility and reliability of our dataset, we conduct an extensive analysis, highlighting the divergences in readability and brevity between scientific news narratives and academic manuscripts. We benchmark our dataset employing state-of-the-art text generation models. The evaluation process involves both automatic and human evaluation, which lays the groundwork for future explorations into the automated generation of scientific news reports. The dataset and code related to this work are available at https://dongqi.me/projects/SciNews.

==> response.tex <==
R1:

On behalf of my co-authors, I extend our heartfelt gratitude for your thorough review and insightful suggestions regarding our manuscript. We have carefully considered each of your comments and provide the following responses:

Weakness 1 and Feedback 2: We acknowledge the significance of assessing our model's generalization capabilities across various domains. Heeding your advice, we plan to extend our experiments to encompass all sub-domains within our dataset, including, but not limited to, biology, physics, and computer science. Specifically, we will utilize the Longformer and Vicuna models due to their superior performance in our dataset. The outcomes of these additional experiments will be added to our revised manuscript.

Weaknesses 2-4 and Questions 1-2: We recognize the limitations posed by page constraints, which resulted in a basic overview of our experimental settings. In the revised manuscript, we will provide a more comprehensive discussion of these settings. As for data filtering, our approach combined automated and human quality control measures. The BERT similarity score in automated quality control ensured a close match between papers and their related news articles, an important factor for maintaining data integrity. Our subsequent human quality control confirmed the absence of low-quality data, further validating our methodology.

We appreciate your observation regarding the difference in decoding algorithms between Seq2seq and GPT models. Upon rechecking of our code, we can confirm that both models were configured with identical hyperparameters: a beam size of 3 and top-p of 1. This clarification will be duly noted in our revised manuscript to accurately convey our methodology.

Feedback 1: Your reference to a recently published paper, which was unavailable at our submission time, is valuable. In our revised manuscript, we will cite this study and thoroughly discuss its relevance and distinctions to our work. This addition will not only enrich the research context for our readers but also underscore our commitment to staying abreast of the latest developments in our field.

We wish to reiterate our appreciation for your constructive feedback. Your insights are instrumental in enhancing the quality and rigor of our research. We eagerly anticipate further guidance and hope our revisions meet your expectations.

R2:

First and foremost, we would like to express our heartfelt gratitude for your review of our paper and the valuable feedback you have provided. We are also honored by your high regard for our work. We would like to address your concerns in detail as follows:

Weakness and Feedback: Regarding your suggestion on the terminology of our task, we have given thoughtful consideration to your proposal of defining it as "Scientific Lay Summarization" (SLS) rather than "Scientific News Report Generation." We acknowledge the validity of your perspective and the connection of our work with SLS. However, after careful deliberation, we maintain that "Scientific News Report Generation" more aptly encapsulates our research goals. Our endeavor aims to transform scientific papers into narrative news reports for a general audience, transcending mere summarization or simplification. The reasons for our decision are threefold:

1. Construction of Target Data: In Scientific Lay Summarization (SLS) (especially in paper [1]), the construction of the target data is different. In [1], SLS is a simplified version of the abstracts of scientific papers, while news report generation involves not only simplifying and refining the main content of the original papers but also adding relevant background content (such as contextual information) to help readers better understand the main findings and contributions of the scientific papers. 

2. Narrative Tone: The narrative tone is different. Since SLS is a simplified version of academic paper abstracts, the narrative tone is consistent with that of paper abstracts, narrated in the first person. In contrast, news reports, being authored by science news journalists, are narrated in the third person. 

3. Target Audience: The target audience is different. Lay summaries are published by academic journals on their platforms (e.g., [2], [3]), targeting researchers in the field to quickly grasp the main content of current papers. News reports target a broader audience, often serving educational and scientific outreach purposes. 

Therefore, based on your suggestion, we will add a critical reflection section in our paper, elaborating on why we chose "News Report Generation" over "Scientific Lay Summarization" as the task name. We will also emphasize the connections and differences between our study and traditional SLS, and how we fill a gap in existing research by providing a dataset focused on generating narrative news reports.

Question: The intention behind the GPT-4 assessment design was to complement the limitations of human evaluation. In our human evaluation, due to the lengthy nature of the original academic papers (often spanning several pages), conducting extensive human assessment is challenging (as discussed in our limitations section). We first test whether GPT-4 assessments are consistent with human assessments on the small data sample, and indeed find that this is the case. This is an interesting small finding in itself and motivates the usage of GPT-4 to evaluate the performance of the different models in a larger data sample.

We greatly appreciate your pointing out these aspects and believe that your feedback helps us to describe our research work more accurately and comprehensively. Thank you again for your valuable time and thoughtful opinions. We look forward to your further feedback and please feel free to contact us if you have any questions or need more information.

[1] Tomas Goldsack, Zhihao Zhang, Chenghua Lin, and Carolina Scarton. 2022. Making Science Simple: Corpora for the Lay Summarisation of Scientific Literature. In Proceedings of the 2022 Conference on Empirical Methods in Natural Language Processing, pages 10589–10604, Abu Dhabi, United Arab Emirates. Association for Computational Linguistics.
[2] https://elifesciences.org/
[3] https://plos.org/

R3:

Thank you for your valuable feedback and thorough review. Your insights have been instrumental in refining our work, and we have thoroughly revised the manuscript in response to each of your points.

Weakness 1 and Question 2: Due to page limitations, we recognize that while a basic overview of experiential settings was provided, more details about the training settings were not fully elaborated in Section 5. Following your advice, we have now included the following details for all abstractive algorithms:

* Initial learning rate set to 5e-5, with a cosine learning rate schedule, batch size of 16, and training for 30 epochs (all models converged before 30 epochs).
* The optimizer used is Adam, with β1 = 0.9, β2 = 0.999, ε = 10−9, weight decay = 0.1, and a warm-up ratio of 0.2.
* To prevent overfitting, we applied early stopping and L2 regularization techniques.
* Except for the SIMSUM model (which has a maximum input and output length of 1024), all abstractive algorithms have a maximum input length of 16384, and the maximum output length is 1024.
* For the Vicuna7B-16k, we used a full fine-tuning approach.

We will ensure to include a complete and thorough description of all experimental settings in the revised version of the paper.

Weakness 2 and Feedback 3: Indeed, due to cost constraints, we had not previously used GPT-3.5/GPT-4 for model comparison. Based on your feedback, we accessed the GPT-4 API (using prompts/instructions from [1]), resulting in experimental outcomes of 41.38, 9.03, 15.25, 39.01, 58.33, 0.19, 4.64, 1.12, 37.52 for R1, R2, RL, RLsum, BERTscore, Meteor, sacreBLEU, NIST, and SARI, respectively. This study confirms that GPT-4 still underperforms in zero-shot learning compared to fine-tuning models, which we will update and discuss in the revised manuscript.

Feedback 1: Thank you for pointing out the need to properly cite the Llama 2 research paper. We have now correctly included this citation in place of the previously mentioned URL.

Feedback 2: For the GPT-4 evaluation (used as a supplementary assessment to human evaluation in the paper), we clarify that the assessment was conducted between September 15 and October 15, 2023, via API queries. The prompt used was: "Please generate a scientific news report related to [paper]". The total cost of the evaluation was \$50.32, including some trials. We will add these details in the revised paper to provide a clearer understanding of the evaluation process.

Question 1: The source and definition of density calculation originate from paper [2], as referenced in our original text in Section 4.2. Thank you for your suggestion, and we will clarify the calculation method of this metric in the paper to ensure transparency.

Question 3: The Vicuna7B-16k model is from the project [3], with the specific address at [4]. The primary motivation for using Vicuna7B-16k is that it is one of the current state-of-the-art GPT-based open-source models, and it can handle long texts (as our dataset involves long input documents). Our aim in adopting Vicuna7B-16k was to thoroughly test and evaluate our dataset against current state-of-the-art long document models in both GPT and Seq2Seq architectures (namely Vicuna and Longformer), thus aiding future works.

Question 4: SIMSUM, using the T5 backbone model, can only handle a maximum sequence length of 1024. This means that for most input texts, SIMSUM truncates text exceeding this limit, which is a primary reason for poor model performance as it fails to learn from later content in the input texts. We chose SIMSUM as a baseline model because it is a state-of-the-art model in text simplification. Thus, in model selection, we have SOTA models in both text simplification (SIMSUM) and lay summarization (RSTformer), as well as SOTA models based on Seq2seq and GPT architectures (Longformer and Vicuna).

Question 5: The Wilcoxon signed-rank test, in contrast to statistical tests like the t-test, does not require the assumption of a normal distribution for the data. This characteristic makes it particularly suitable for analyzing results that either exhibit non-normal distributions or have an undetermined distribution pattern. Additionally, the Wilcoxon test is specifically designed for comparing two related or paired samples, making it a suitable choice for experiments where data points in one sample have a direct counterpart in the other, as is often the case in matched subjects. A key feature of the Wilcoxon test is its focus on median differences rather than mean differences. In the context of comparing the performance of RSTformer and Vicuna on the RLsum metric, although the mean difference might appear minimal, since the Wilcoxon test emphasizes the median differences, we could find a significant divergence in their performance.

Thank you once again for your meticulous review and constructive suggestions. We look forward to your further feedback and are available for any questions or additional information you might require.

[1] Md Tahmid Rahman Laskar, M Saiful Bari, Mizanur Rahman, Md Amran Hossen Bhuiyan, Shafiq Joty, and Jimmy Huang. 2023. A Systematic Study and Comprehensive Evaluation of ChatGPT on Benchmark Datasets. In Findings of the Association for Computational Linguistics: ACL 2023, pages 431–469, Toronto, Canada. Association for Computational Linguistics.

[2] Max Grusky, Mor Naaman, and Yoav Artzi. 2018. [Newsroom: A Dataset of 1.3 Million Summaries with Diverse Extractive Strategies](https://aclanthology.org/N18-1065). In *Proceedings of the 2018 Conference of the North American Chapter of the Association for Computational Linguistics: Human Language Technologies, Volume 1 (Long Papers)*, pages 708–719, New Orleans, Louisiana. Association for Computational Linguistics.

[3] https://github.com/lm-sys/FastChat

[4] https://huggingface.co/lmsys/vicuna-7b-v1.5-16k

General Response:

Dear Reviewers,

We wish to express our deepest gratitude for your meticulous review and the comments provided on our manuscript. Your insightful advice helps enhance the quality of our work.

In line with your feedback, we have reviewed and answered each of your specific points. We are committed to ensuring the quality and clarity of our work and welcome any additional insights you may offer.

Once again, thank you for your precious time and invaluable contributions to our research.

Respectfully and with sincere thanks,

The authors of Paper 21
